Iterative Deepening Hyperband

Hyperparameter optimization (HPO) is concerned with the automated search for the most appropriate hyperparameter configuration (HPC) of a parameterized machine learning algorithm. A state-of-the-art HPO method is Hyperband, which, however, has its own parameters that influence its performance. One of these parameters, the maximal budget, is especially problematic: If chosen too small, the budget needs to be increased in hindsight and, as Hyperband is not incremental by design, the entire algorithm must be re-run. This is not only costly but also comes with a loss of valuable knowledge already accumulated. In this paper, we propose incremental variants of Hyperband that eliminate these drawbacks, and show that these variants satisfy theoretical guarantees qualitatively similar to those for the original Hyperband with the "right" budget. Moreover, we demonstrate their practical utility in experiments with benchmark data sets.

==> idsh.tex <==
%% actually not needed anymore since it is already integrated with HB in the main tex file

\begin{algorithm*}\caption{IterativeDeepening-SuccessiveHalving (ID-SH)}


\begin{algorithmic}
\Require $\eta, r, R, \text{promoted}^{(i)}, \text{unpromoted}^{(i)}, \text{new\_candidates}$
\State candidates\_to\_promote $\gets$ new\_candidates
\For{$i \in \{ r, \ldots, \log_\eta(R) \}$}
    \State $\text{evaluate}(\text{candidates\_to\_promote}, r \eta^i)$
    \State $\text{n\_promote} \gets (|\text{promoted}^{(i)}| + |\text{unpromoted}^{(i)}| + |\text{candidates\_to\_promote}|) \eta^{-1} - |\text{promoted}^{(i)}|$
    % compute top k for the remaining promotions (n_promote)
    \State $\text{promotion\_candidates} \gets \text{unpromoted}^{(i)} \cup \text{candidates\_to\_promote}$
    \State $\text{candidates\_to\_promote} \gets \text{top}_{\text{n\_promote}}(\text{promotion\_candidates})$

    \State $\text{promoted}^{(i)} \gets \text{promoted}^{(i)} \cup \text{candidates\_to\_promote}$
    \State $\text{unpromoted}^{(i)} \gets \text{promotion\_candidates} \setminus \text{candidates\_to\_promote}$
\EndFor
\State \Return $\text{top}_1(\text{promoted}^{(\log_\eta(R))})$
\end{algorithmic}
\end{algorithm*}

==> table_idhb.tex <==
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
3945 & .993$\pm$.00 & .993$\pm$.00 & .993$\pm$.00 & .993$\pm$.00\\
7593 & .716$\pm$.03 & .716$\pm$.03 & .716$\pm$.03 & .716$\pm$.03\\
34539 & .981$\pm$.01 & .981$\pm$.01 & .981$\pm$.01 & .981$\pm$.01\\
126025 & .881$\pm$.02 & .881$\pm$.02 & .879$\pm$.02 & .877$\pm$.02\\
126026 & .966$\pm$.01 & .966$\pm$.01 & .966$\pm$.01 & .965$\pm$.01\\
126029 & .926$\pm$.01 & .926$\pm$.01 & .926$\pm$.01 & .926$\pm$.01\\
146212 & .975$\pm$.01 & .975$\pm$.01 & .976$\pm$.01 & .975$\pm$.01\\
167104 & .922$\pm$.01 & .922$\pm$.01 & .922$\pm$.01 & .922$\pm$.01\\
167149 & .971$\pm$.00 & .971$\pm$.00 & .971$\pm$.00 & .970$\pm$.00\\
167152 & .967$\pm$.00 & .967$\pm$.00 & .967$\pm$.00 & .967$\pm$.00\\
167161 & .818$\pm$.03 & .818$\pm$.03 & .818$\pm$.03 & .816$\pm$.03\\
167168 & .780$\pm$.02 & .780$\pm$.02 & .780$\pm$.02 & .779$\pm$.02\\
167181 & .904$\pm$.01 & .904$\pm$.01 & .904$\pm$.01 & .903$\pm$.01\\
167184 & .800$\pm$.01 & .800$\pm$.01 & .800$\pm$.01 & .800$\pm$.02\\
167185 & .961$\pm$.00 & .961$\pm$.00 & .961$\pm$.00 & .961$\pm$.00\\
167190 & .847$\pm$.01 & .847$\pm$.01 & .847$\pm$.01 & .845$\pm$.01\\
167200 & .715$\pm$.02 & .715$\pm$.02 & .715$\pm$.02 & .713$\pm$.02\\
167201 & .738$\pm$.04 & .738$\pm$.04 & .738$\pm$.04 & .738$\pm$.04\\
168329 & .281$\pm$.03 & .281$\pm$.03 & .279$\pm$.03 & .277$\pm$.03\\
168330 & .636$\pm$.02 & .636$\pm$.02 & .637$\pm$.02 & .637$\pm$.02\\
168331 & .582$\pm$.04 & .582$\pm$.04 & .582$\pm$.04 & .582$\pm$.04\\
168335 & .929$\pm$.01 & .929$\pm$.01 & .929$\pm$.01 & .929$\pm$.01\\
168868 & .996$\pm$.00 & .996$\pm$.00 & .996$\pm$.00 & .996$\pm$.00\\
168908 & .814$\pm$.01 & .814$\pm$.01 & .815$\pm$.01 & .815$\pm$.01\\
168910 & .675$\pm$.02 & .675$\pm$.02 & .675$\pm$.02 & .675$\pm$.02\\
189354 & .704$\pm$.03 & .704$\pm$.03 & .704$\pm$.03 & .704$\pm$.03\\
189862 & .852$\pm$.02 & .852$\pm$.02 & .853$\pm$.02 & .852$\pm$.02\\
189865 & .944$\pm$.01 & .944$\pm$.01 & .944$\pm$.01 & .944$\pm$.01\\
189866 & .690$\pm$.03 & .690$\pm$.03 & .690$\pm$.03 & .690$\pm$.03\\
189873 & .797$\pm$.03 & .797$\pm$.03 & .797$\pm$.03 & .797$\pm$.03\\
189905 & .905$\pm$.02 & .905$\pm$.02 & .905$\pm$.02 & .905$\pm$.02\\
189906 & .865$\pm$.02 & .865$\pm$.02 & .865$\pm$.02 & .865$\pm$.02\\
189908 & .872$\pm$.01 & .872$\pm$.01 & .872$\pm$.01 & .872$\pm$.01\\
189909 & .752$\pm$.02 & .752$\pm$.02 & .753$\pm$.02 & .753$\pm$.02\\
\end{tabular}
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
3945 & .993$\pm$.00 & .993$\pm$.00 & .993$\pm$.00 & .993$\pm$.00\\
7593 & .711$\pm$.04 & .711$\pm$.04 & .711$\pm$.04 & .712$\pm$.04\\
34539 & .982$\pm$.01 & .982$\pm$.01 & .982$\pm$.01 & .982$\pm$.01\\
126025 & .886$\pm$.02 & .886$\pm$.02 & .887$\pm$.02 & .888$\pm$.02\\
126026 & .965$\pm$.01 & .965$\pm$.01 & .965$\pm$.01 & .965$\pm$.01\\
126029 & .923$\pm$.02 & .923$\pm$.02 & .924$\pm$.02 & .924$\pm$.02\\
146212 & .975$\pm$.01 & .975$\pm$.01 & .975$\pm$.01 & .975$\pm$.01\\
167104 & .922$\pm$.01 & .922$\pm$.01 & .922$\pm$.01 & .922$\pm$.01\\
167149 & .969$\pm$.01 & .969$\pm$.01 & .969$\pm$.01 & .969$\pm$.01\\
167152 & .967$\pm$.00 & .967$\pm$.00 & .967$\pm$.00 & .967$\pm$.00\\
167161 & .821$\pm$.03 & .821$\pm$.03 & .822$\pm$.03 & .816$\pm$.03\\
167168 & .770$\pm$.02 & .770$\pm$.02 & .770$\pm$.02 & .770$\pm$.02\\
167181 & .903$\pm$.02 & .903$\pm$.02 & .903$\pm$.02 & .903$\pm$.02\\
167184 & .798$\pm$.03 & .798$\pm$.03 & .799$\pm$.03 & .796$\pm$.03\\
167185 & .961$\pm$.00 & .961$\pm$.00 & .961$\pm$.00 & .961$\pm$.00\\
167190 & .851$\pm$.02 & .851$\pm$.02 & .853$\pm$.01 & .848$\pm$.02\\
167200 & .710$\pm$.02 & .710$\pm$.02 & .710$\pm$.02 & .711$\pm$.02\\
167201 & .735$\pm$.05 & .735$\pm$.05 & .736$\pm$.05 & .736$\pm$.05\\
168329 & .273$\pm$.04 & .273$\pm$.04 & .273$\pm$.04 & .273$\pm$.04\\
168330 & .635$\pm$.03 & .635$\pm$.03 & .635$\pm$.03 & .635$\pm$.03\\
168331 & .562$\pm$.05 & .562$\pm$.05 & .562$\pm$.05 & .562$\pm$.05\\
168335 & .926$\pm$.02 & .926$\pm$.02 & .926$\pm$.02 & .926$\pm$.02\\
168868 & .996$\pm$.00 & .996$\pm$.00 & .996$\pm$.00 & .996$\pm$.00\\
168908 & .808$\pm$.01 & .808$\pm$.01 & .808$\pm$.02 & .808$\pm$.02\\
168910 & .682$\pm$.03 & .682$\pm$.03 & .682$\pm$.03 & .682$\pm$.03\\
189354 & .706$\pm$.03 & .706$\pm$.03 & .706$\pm$.03 & .706$\pm$.03\\
189862 & .856$\pm$.02 & .856$\pm$.02 & .856$\pm$.02 & .854$\pm$.02\\
189865 & .943$\pm$.01 & .943$\pm$.01 & .943$\pm$.01 & .943$\pm$.01\\
189866 & .686$\pm$.03 & .686$\pm$.03 & .686$\pm$.03 & .686$\pm$.03\\
189873 & .771$\pm$.08 & .771$\pm$.08 & .771$\pm$.08 & .771$\pm$.08\\
189905 & .898$\pm$.02 & .898$\pm$.02 & .898$\pm$.02 & .898$\pm$.02\\
189906 & .860$\pm$.02 & .860$\pm$.02 & .860$\pm$.02 & .860$\pm$.02\\
189908 & .871$\pm$.02 & .871$\pm$.02 & .871$\pm$.02 & .871$\pm$.02\\
189909 & .747$\pm$.03 & .747$\pm$.03 & .748$\pm$.03 & .748$\pm$.03\\
\end{tabular}
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
CIFAR10 & .906$\pm$.00 & .906$\pm$.00 & .906$\pm$.00 & .906$\pm$.00\\
\end{tabular}
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
CIFAR10 & .939$\pm$.00 & .939$\pm$.00 & .939$\pm$.00 & .939$\pm$.00\\
\end{tabular}
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
3 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
6 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
11 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
12 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
14 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
15 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
16 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
18 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
22 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
24 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
28 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
29 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
31 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
32 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
37 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
38 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
42 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
44 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
46 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
50 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
54 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
60 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
151 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
181 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
182 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
188 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
300 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
307 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
312 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
334 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
375 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
377 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
458 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
469 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00\\
470 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
554 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1040 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1049 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1050 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1053 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1056 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1063 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1067 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1068 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1111 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1220 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1457 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1461 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1462 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1464 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1468 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1475 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
1476 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1478 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1479 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
1480 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1485 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1486 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1487 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1489 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1493 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1494 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1497 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1501 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1510 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1515 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1590 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4134 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
4135 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4154 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4534 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4538 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
4541 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
6332 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23381 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
23512 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23517 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
40496 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40498 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40499 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40536 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40668 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40670 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40685 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40701 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40900 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40923 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40927 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40966 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40975 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40978 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40979 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40981 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40982 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40983 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40984 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40994 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40996 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41027 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41138 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41142 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41143 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41146 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41150 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41156 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41157 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41159 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41161 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41162 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41163 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41164 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41165 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41166 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41168 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41169 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41212 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41216 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00\\
41278 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
\end{tabular}
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
3 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
6 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
11 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
12 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
14 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
15 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
16 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
18 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
22 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
24 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
28 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
29 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
31 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
32 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
37 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
38 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
42 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
44 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
46 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
50 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
54 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
60 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
151 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
181 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
182 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
188 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
300 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
307 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
312 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
334 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
375 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
377 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
458 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
469 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00\\
470 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
554 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1040 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1049 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1050 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1053 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1056 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1063 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1067 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1068 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1111 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1220 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1457 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1461 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1462 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1464 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1468 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1475 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
1476 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1478 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1479 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
1480 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1485 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1486 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1487 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1489 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1493 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1494 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1497 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1501 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1510 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1515 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1590 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4134 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
4135 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4154 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4534 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4538 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
4541 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
6332 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23381 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
23512 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23517 & .005$\pm$.00 & .005$\pm$.00 & .005$\pm$.00 & .005$\pm$.00\\
40496 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40498 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40499 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40536 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40668 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40670 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40685 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40701 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40900 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40923 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40927 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40966 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40975 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40978 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40979 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40981 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40982 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40983 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40984 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40994 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40996 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41027 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41138 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41142 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41143 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41146 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41150 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41156 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41157 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41159 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41161 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41162 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41163 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41164 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41165 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41166 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41168 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41169 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
41212 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41216 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00\\
41278 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
\end{tabular}
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
3 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
6 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
11 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
12 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
14 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
15 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
16 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
18 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
22 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
23 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
24 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
28 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
29 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
31 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
32 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
37 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
38 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
42 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
44 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
46 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
50 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
54 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
60 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
151 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
181 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
182 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
188 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
300 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
307 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
312 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
334 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
375 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
377 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
458 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
469 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00\\
470 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1040 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1049 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1050 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1053 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1056 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1063 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1067 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1068 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1111 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1220 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1457 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1461 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1462 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1464 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1468 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1475 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
1476 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1478 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1479 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1480 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1485 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
1486 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1487 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1489 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1493 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1494 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1497 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1501 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1510 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1515 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1590 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4134 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
4135 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4154 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4534 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4538 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
6332 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23381 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
40496 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40498 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40499 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40536 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40668 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40670 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40685 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40701 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40900 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40966 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40975 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40978 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40979 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40981 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40982 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40983 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40984 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40994 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41027 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41138 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41142 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41143 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41146 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41156 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41157 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41162 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41163 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41164 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41169 & .004$\pm$.00 & .004$\pm$.00 & .004$\pm$.00 & .004$\pm$.00\\
41212 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41216 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00\\
41278 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
\end{tabular}
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
3 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
6 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
11 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
12 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
14 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
15 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
16 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
18 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
22 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
23 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
24 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
28 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
29 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
31 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
32 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
37 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
38 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
42 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
44 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
46 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
50 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
54 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
60 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
151 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
181 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
182 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
188 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
300 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
307 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
312 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
334 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
375 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
377 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
458 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
469 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00\\
470 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1040 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1049 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1050 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1053 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1056 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1063 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1067 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1068 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1111 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1220 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1457 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1461 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1462 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1464 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1468 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1475 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
1476 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1478 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1479 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1480 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1485 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
1486 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1487 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1489 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1493 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1494 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1497 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1501 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1510 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1515 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1590 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4134 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
4135 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4154 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4534 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4538 & .005$\pm$.00 & .005$\pm$.00 & .005$\pm$.00 & .005$\pm$.00\\
6332 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23381 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
40496 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40498 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40499 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40536 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40668 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40670 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40685 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40701 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40900 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40966 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40975 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40978 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40979 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40981 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40982 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40983 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40984 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40994 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41027 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41138 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41142 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41143 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41146 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41156 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41157 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41162 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41163 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41164 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
41169 & .004$\pm$.00 & .004$\pm$.00 & .004$\pm$.00 & .004$\pm$.00\\
41212 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41216 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00\\
41278 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
\end{tabular}
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
3 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
6 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
11 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
12 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
14 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
15 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
16 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
18 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
22 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
23 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
24 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
28 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
29 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
31 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
32 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
37 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
38 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
42 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
44 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
46 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
50 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
54 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
60 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
151 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
181 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
182 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
188 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
300 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
307 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
312 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
334 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
375 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
377 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
458 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
469 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00 & .003$\pm$.00\\
470 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
554 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1040 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1049 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1050 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1053 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1056 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1063 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1067 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1068 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1111 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1220 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1457 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1461 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1462 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1464 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1468 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1475 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1476 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1478 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1479 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1480 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1485 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1486 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1487 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1489 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1493 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1494 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1497 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1501 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1510 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1515 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1590 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4134 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
4135 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4154 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4534 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4538 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4541 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
6332 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23381 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
23512 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
23517 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40496 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40498 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40499 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40536 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40668 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40670 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40685 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40701 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40900 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40923 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40927 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40966 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40975 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40978 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40979 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40981 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40982 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40983 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40984 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40994 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40996 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41027 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41138 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41142 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41143 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41146 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41150 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41156 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41157 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41159 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41161 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41162 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41163 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41164 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41165 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41166 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41168 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41169 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41212 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41216 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41278 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
\end{tabular}
\begin{tabular}{lllll}&0ih-hb&1dcid-hb&2cid-hb&3eid-hb\\
3 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
6 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
11 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
12 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
14 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
15 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
16 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
18 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
22 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
24 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
28 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
29 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
31 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
32 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
37 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
38 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
42 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
44 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
46 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
50 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
54 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
60 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
151 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
181 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
182 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
188 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
300 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
307 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
312 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
334 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
375 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
377 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
458 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
469 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00 & .002$\pm$.00\\
470 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
554 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1040 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1049 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1050 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1053 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1056 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1063 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1067 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1068 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1111 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1220 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1457 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1461 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1462 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1464 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1468 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1475 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
1476 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1478 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1479 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1480 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1485 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
1486 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1487 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1489 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1493 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1494 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1497 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1501 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
1510 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
1515 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
1590 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4134 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
4135 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
4154 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4534 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
4538 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
4541 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
6332 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
23381 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00 & .006$\pm$.00\\
23512 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
23517 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40496 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40498 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00 & .007$\pm$.00\\
40499 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40536 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40668 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40670 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40685 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40701 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40900 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40923 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40927 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40966 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40975 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40978 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40979 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40981 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40982 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
40983 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40984 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
40994 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
40996 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41027 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41138 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41142 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41143 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41146 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41150 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41156 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41157 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41159 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41161 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41162 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41163 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41164 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41165 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41166 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41168 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41169 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
41212 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00 & .008$\pm$.00\\
41216 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00 & .009$\pm$.00\\
41278 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00 & .010$\pm$.00\\
\end{tabular}


==> table_yahpo_lcbench_2.tex <==
\begin{tabular}{lllll}
\toprule
OpenML ID&\baselinehb&\discardingidhb&\conservativehb&\efficienthb\\
\midrule
3945 & .993$\pm$.00 & .993$\pm$.00 & .993$\pm$.00 & .993$\pm$.00\\
7593 & .716$\pm$.03 & .716$\pm$.03 & .716$\pm$.03 & .716$\pm$.03\\
34539 & .981$\pm$.01 & .981$\pm$.01 & .981$\pm$.01 & .981$\pm$.01\\
126025 & .881$\pm$.02 & .881$\pm$.02 & .879$\pm$.02 & .877$\pm$.02\\
126026 & .966$\pm$.01 & .966$\pm$.01 & .966$\pm$.01 & .965$\pm$.01\\
126029 & .926$\pm$.01 & .926$\pm$.01 & .926$\pm$.01 & .926$\pm$.01\\
146212 & .975$\pm$.01 & .975$\pm$.01 & .976$\pm$.01 & .975$\pm$.01\\
167104 & .922$\pm$.01 & .922$\pm$.01 & .922$\pm$.01 & .922$\pm$.01\\
167149 & .971$\pm$.00 & .971$\pm$.00 & .971$\pm$.00 & .970$\pm$.00\\
167152 & .967$\pm$.00 & .967$\pm$.00 & .967$\pm$.00 & .967$\pm$.00\\
167161 & .818$\pm$.03 & .818$\pm$.03 & .818$\pm$.03 & .816$\pm$.03\\
167168 & .780$\pm$.02 & .780$\pm$.02 & .780$\pm$.02 & .779$\pm$.02\\
167181 & .904$\pm$.01 & .904$\pm$.01 & .904$\pm$.01 & .903$\pm$.01\\
167184 & .800$\pm$.01 & .800$\pm$.01 & .800$\pm$.01 & .800$\pm$.02\\
167185 & .961$\pm$.00 & .961$\pm$.00 & .961$\pm$.00 & .961$\pm$.00\\
167190 & .847$\pm$.01 & .847$\pm$.01 & .847$\pm$.01 & .845$\pm$.01\\
167200 & .715$\pm$.02 & .715$\pm$.02 & .715$\pm$.02 & .713$\pm$.02\\
167201 & .738$\pm$.04 & .738$\pm$.04 & .738$\pm$.04 & .738$\pm$.04\\
168329 & .281$\pm$.03 & .281$\pm$.03 & .279$\pm$.03 & .277$\pm$.03\\
168330 & .636$\pm$.02 & .636$\pm$.02 & .637$\pm$.02 & .637$\pm$.02\\
168331 & .582$\pm$.04 & .582$\pm$.04 & .582$\pm$.04 & .582$\pm$.04\\
168335 & .929$\pm$.01 & .929$\pm$.01 & .929$\pm$.01 & .929$\pm$.01\\
168868 & .996$\pm$.00 & .996$\pm$.00 & .996$\pm$.00 & .996$\pm$.00\\
168908 & .814$\pm$.01 & .814$\pm$.01 & .815$\pm$.01 & .815$\pm$.01\\
168910 & .675$\pm$.02 & .675$\pm$.02 & .675$\pm$.02 & .675$\pm$.02\\
189354 & .704$\pm$.03 & .704$\pm$.03 & .704$\pm$.03 & .704$\pm$.03\\
189862 & .852$\pm$.02 & .852$\pm$.02 & .853$\pm$.02 & .852$\pm$.02\\
189865 & .944$\pm$.01 & .944$\pm$.01 & .944$\pm$.01 & .944$\pm$.01\\
189866 & .690$\pm$.03 & .690$\pm$.03 & .690$\pm$.03 & .690$\pm$.03\\
189873 & .797$\pm$.03 & .797$\pm$.03 & .797$\pm$.03 & .797$\pm$.03\\
189905 & .905$\pm$.02 & .905$\pm$.02 & .905$\pm$.02 & .905$\pm$.02\\
189906 & .865$\pm$.02 & .865$\pm$.02 & .865$\pm$.02 & .865$\pm$.02\\
189908 & .872$\pm$.01 & .872$\pm$.01 & .872$\pm$.01 & .872$\pm$.01\\
189909 & .752$\pm$.02 & .752$\pm$.02 & .753$\pm$.02 & .753$\pm$.02\\
\bottomrule
\end{tabular}

==> table_yahpo_lcbench_3.tex <==
\begin{tabular}{lllll}
\toprule
OpenML ID&\baselinehb&\discardingidhb&\conservativeidhb&\efficientidhb\\
\midrule
3945 & .993$\pm$.00 & .993$\pm$.00 & .993$\pm$.00 & .993$\pm$.00\\
7593 & .711$\pm$.04 & .711$\pm$.04 & .711$\pm$.04 & .712$\pm$.04\\
34539 & .982$\pm$.01 & .982$\pm$.01 & .982$\pm$.01 & .982$\pm$.01\\
126025 & .886$\pm$.02 & .886$\pm$.02 & .887$\pm$.02 & .888$\pm$.02\\
126026 & .965$\pm$.01 & .965$\pm$.01 & .965$\pm$.01 & .965$\pm$.01\\
126029 & .923$\pm$.02 & .923$\pm$.02 & .924$\pm$.02 & .924$\pm$.02\\
146212 & .975$\pm$.01 & .975$\pm$.01 & .975$\pm$.01 & .975$\pm$.01\\
167104 & .922$\pm$.01 & .922$\pm$.01 & .922$\pm$.01 & .922$\pm$.01\\
167149 & .969$\pm$.01 & .969$\pm$.01 & .969$\pm$.01 & .969$\pm$.01\\
167152 & .967$\pm$.00 & .967$\pm$.00 & .967$\pm$.00 & .967$\pm$.00\\
167161 & .821$\pm$.03 & .821$\pm$.03 & .822$\pm$.03 & .816$\pm$.03\\
167168 & .770$\pm$.02 & .770$\pm$.02 & .770$\pm$.02 & .770$\pm$.02\\
167181 & .903$\pm$.02 & .903$\pm$.02 & .903$\pm$.02 & .903$\pm$.02\\
167184 & .798$\pm$.03 & .798$\pm$.03 & .799$\pm$.03 & .796$\pm$.03\\
167185 & .961$\pm$.00 & .961$\pm$.00 & .961$\pm$.00 & .961$\pm$.00\\
167190 & .851$\pm$.02 & .851$\pm$.02 & .853$\pm$.01 & .848$\pm$.02\\
167200 & .710$\pm$.02 & .710$\pm$.02 & .710$\pm$.02 & .711$\pm$.02\\
167201 & .735$\pm$.05 & .735$\pm$.05 & .736$\pm$.05 & .736$\pm$.05\\
168329 & .273$\pm$.04 & .273$\pm$.04 & .273$\pm$.04 & .273$\pm$.04\\
168330 & .635$\pm$.03 & .635$\pm$.03 & .635$\pm$.03 & .635$\pm$.03\\
168331 & .562$\pm$.05 & .562$\pm$.05 & .562$\pm$.05 & .562$\pm$.05\\
168335 & .926$\pm$.02 & .926$\pm$.02 & .926$\pm$.02 & .926$\pm$.02\\
168868 & .996$\pm$.00 & .996$\pm$.00 & .996$\pm$.00 & .996$\pm$.00\\
168908 & .808$\pm$.01 & .808$\pm$.01 & .808$\pm$.02 & .808$\pm$.02\\
168910 & .682$\pm$.03 & .682$\pm$.03 & .682$\pm$.03 & .682$\pm$.03\\
189354 & .706$\pm$.03 & .706$\pm$.03 & .706$\pm$.03 & .706$\pm$.03\\
189862 & .856$\pm$.02 & .856$\pm$.02 & .856$\pm$.02 & .854$\pm$.02\\
189865 & .943$\pm$.01 & .943$\pm$.01 & .943$\pm$.01 & .943$\pm$.01\\
189866 & .686$\pm$.03 & .686$\pm$.03 & .686$\pm$.03 & .686$\pm$.03\\
189873 & .771$\pm$.08 & .771$\pm$.08 & .771$\pm$.08 & .771$\pm$.08\\
189905 & .898$\pm$.02 & .898$\pm$.02 & .898$\pm$.02 & .898$\pm$.02\\
189906 & .860$\pm$.02 & .860$\pm$.02 & .860$\pm$.02 & .860$\pm$.02\\
189908 & .871$\pm$.02 & .871$\pm$.02 & .871$\pm$.02 & .871$\pm$.02\\
189909 & .747$\pm$.03 & .747$\pm$.03 & .748$\pm$.03 & .748$\pm$.03\\
\bottomrule
\end{tabular}

